CausalKANs: interpretable treatment effect estimation with Kolmogorov-Arnold networks

Deep neural networks achieve state-of-the-art performance in estimating heterogeneous treatment effects, but their opacity limits trust and adoption in sensitive domains such as medicine, economics, and public policy. Building on well-established and high-performing causal neural architectures, we propose causalKANs, a framework that transforms neural estimators of conditional average treatment effects (CATEs) into Kolmogorov--Arnold Networks (KANs). By incorporating pruning and symbolic simplification, causalKANs yields interpretable closed-form formulas while preserving predictive accuracy. Experiments on benchmark datasets demonstrate that causalKANs perform on par with neural baselines in CATE error metrics, and that even simple KAN variants achieve competitive performance, offering a favorable accuracy--interpretability trade-off. By combining reliability with analytic accessibility, causalKANs provide auditable estimators supported by closed-form expressions and interpretable plots, enabling trustworthy individualized decision-making in high-stakes settings. We release the code for reproducibility at https://github.com/aalmodovares/causalkans .

==> math_commands.tex <==
\RequirePackage{mathtools}
\RequirePackage{amsmath,amsfonts,bm}
\RequirePackage{suffix}

% punctuation of equations, see for example the first answer in
% https://www.reddit.com/r/LaTeX/comments/5xnzg7/correct_grammar_for_putting_an_equation/
\newcommand{\equationPunctuation}[1]{\,{#1}}

%% Bold greek letters
\newcommand{\thetab}{{\boldsymbol{\theta}}}
\newcommand{\betab}{{\boldsymbol{\beta}}}
\newcommand{\pib}{{\boldsymbol{\pi}}}
\newcommand{\taub}{{\boldsymbol{\tau}}}
\newcommand{\psib}{{\boldsymbol{\psi}}}
\newcommand{\phib}{{\boldsymbol{\phi}}}
\newcommand{\omegab}{{\boldsymbol{\omega}}}
\newcommand{\etab}{{\boldsymbol{\eta}}}
\newcommand{\sigmab}{{\boldsymbol{\sigma}}}
\newcommand{\epsilonb}{{\boldsymbol{\epsilon}}}

\newcommand{\Thetab}{{\boldsymbol{\Theta}}}

\newcommand{\distribution}[1][]{\ensuremath{{P}_{#1}}\xspace}
\newcommand{\cumulative}[1][]{\ensuremath{F_{#1}}\xspace}
\newcommand{\empcumulative}[1][]{\ensuremath{\hat F_{#1}}\xspace}
\newcommand{\pushforward}[2]{{#1}_{\#} {#2}}

\DeclareMathOperator{\E}{\mathbb{E}}
\DeclarePairedDelimiter{\Ebrackets}{[}{]}
\newcommand{\Expect}[2][]{\E_{#1}\Ebrackets{#2}}
\WithSuffix\newcommand\Expect*[2][]{\E_{#1}\Ebrackets*{#2}}

\DeclareMathOperator{\V}{\mathbb{V}}
\newcommand{\Var}[2][]{\V_{#1}\Ebrackets{#2}}

\newcommand{\normal}{\ensuremath{\mathcal{N}}\xspace}
\newcommand{\uniform}{\ensuremath{\mathcal{U}}\xspace}
\newcommand{\categorical}{\ensuremath{\operatorname{Cat}}\xspace}
\newcommand{\bernoulli}{\ensuremath{\operatorname{Bern}}\xspace}
\newcommand{\binomial}{\ensuremath{\operatorname{Bin}}\xspace}
\newcommand{\lognormal}{\ensuremath{\operatorname{Log-normal}}\xspace}
\newcommand{\poisson}{\ensuremath{\operatorname{Poiss}}\xspace}
\newcommand{\exponentialdistribution}{\ensuremath{\operatorname{Exp}}\xspace}
\newcommand{\betadistribution}{\ensuremath{\operatorname{Beta}}\xspace}
\newcommand{\weibulldistribution}{\ensuremath{\operatorname{Weibull}}\xspace}

\newcommand{\identity}{\ensuremath{\mI}}
\newcommand{\indicator}[1]{\ensuremath{\mathbf{1}_{\{#1\}}}}
\newcommand{\ones}{\ensuremath{\mathbf{1}}\xspace}
\newcommand{\zeroes}{\ensuremath{\mathbf{0}}\xspace}

\DeclareMathOperator*{\avg}{avg}
\DeclareMathOperator*{\med}{med}
\DeclareMathOperator*{\std}{std}

\let\cossim\cos

%%%%%%

\usepackage{suffix}
\usepackage{xparse}
\usepackage{mathtools}

%%%%
\def\rL{{\textnormal{L}}}
\def\rvL{{\mathbf{L}}}
\def\ervL{{\textnormal{L}}}

\def\rM{{\textnormal{M}}}
\def\rvM{{\mathbf{M}}}
\def\ervM{{\textnormal{M}}}

\def\vT{\bm{T}}
\def\vF{\bm{F}}
\def\vR{\bm{R}}
\def\vU{\bm{U}}
\def\rU{{\textnormal{U}}}
\def\rvU{{\mathbf{U}}}
\def\ervU{{\textnormal{U}}}
%%%%

\newcommand{\tensor}[1]{\ensuremath{\mathsf{#1}}}
\renewcommand{\vec}{\operatorname{vec}}
\newcommand{\D}{\mathrm{D}}
\newcommand{\Gmat}{\mathrm{G}}
\newcommand{\F}{\mathrm{F}}
\newcommand{\He}{\mathrm{H}}
\newcommand{\HeCal}{\mathcal{H}}
%\newcommand{\diff}{\mathrm{d}}
\newcommand*\dif{\mathop{}\!\mathrm{d}}
\newcommand{\average}[1]{\overline{ #1 }}

\newcommand{\Loss}{\mathcal{L}}
\newcommand{\jac}{\mathrm{J}}
\newcommand{\lin}[1]{\left\langle #1 \right\rangle}

\newcommand{\nablasquaredsub}[1]{
  \nabla^{\kern -.0em \raise.1em\hbox{\tiny$2$}} {\kern -.6em \raise-.1em\hbox{\tiny$#1$}}{}
}
\newcommand{\nablasub}[1]{
  \nabla {\kern -.2em \raise-.1em\hbox{\tiny$#1$}}{}
}

% Mark sections of captions for referring to divisions of figures
\newcommand{\figleft}{{\em (Left)}\xspace}
\newcommand{\figcenter}{{\em (Center)}}
\newcommand{\figright}{{\em (Right)}\xspace}
\newcommand{\figtop}{{\em (Top)}}
\newcommand{\figbottom}{{\em (Bottom)}}
\newcommand{\captiona}{{\bfseries \color{maincolor} (a)}\xspace}
\newcommand{\captionb}{{\bfseries \color{maincolor}  (b)}\xspace}
\newcommand{\captionc}{{\bfseries \color{maincolor}  (c)}\xspace}
\newcommand{\captiond}{{\bfseries \color{maincolor}  (d)}\xspace}


% Added by me (@Adrian) to be consinstent when I do listings
\newcommand{\itemi}{{\bfseries \color{maincolor} i)}\xspace}
\newcommand{\itemii}{{\bfseries \color{maincolor} ii)}\xspace}
\newcommand{\itemiii}{{\bfseries \color{maincolor} iii)}\xspace}
\newcommand{\itemiv}{{\bfseries \color{maincolor} iv)}\xspace}
\newcommand{\itemv}{{\bfseries \color{maincolor} v)}\xspace}
\newcommand{\itemvi}{{\bfseries \color{maincolor} vi)}\xspace}
\newcommand{\itemvii}{{\bfseries \color{maincolor} vii)}\xspace}

% Highlight a newly defined term
\newcommand{\newterm}[1]{{\bf #1}}

% Figure reference, lower-case.
\def\figref#1{figure~\ref{#1}}
% Figure reference, capital. For start of sentence
\def\Figref#1{Figure~\ref{#1}}
\def\twofigref#1#2{figures \ref{#1} and \ref{#2}}
\def\quadfigref#1#2#3#4{figures \ref{#1}, \ref{#2}, \ref{#3} and \ref{#4}}
% Section reference, lower-case.
\def\secref#1{section~\ref{#1}}
% Section reference, capital.
\def\Secref#1{Section~\ref{#1}}
% Reference to two sections.
\def\twosecrefs#1#2{sections \ref{#1} and \ref{#2}}
% Reference to three sections.
\def\secrefs#1#2#3{sections \ref{#1}, \ref{#2} and \ref{#3}}
% Reference to an equation, lower-case.
\def\eqref#1{equation~\ref{#1}}
% Reference to an equation, upper case
\def\Eqref#1{Equation~\ref{#1}}
% A raw reference to an equation---avoid using if possible
\def\plaineqref#1{\ref{#1}}
% Reference to a chapter, lower-case.
\def\chapref#1{chapter~\ref{#1}}
% Reference to an equation, upper case.
\def\Chapref#1{Chapter~\ref{#1}}
% Reference to a range of chapters
\def\rangechapref#1#2{chapters\ref{#1}--\ref{#2}}
% Reference to an algorithm, lower-case.
\def\algref#1{algorithm~\ref{#1}}
% Reference to an algorithm, upper case.
\def\Algref#1{Algorithm~\ref{#1}}
\def\twoalgref#1#2{algorithms \ref{#1} and \ref{#2}}
\def\Twoalgref#1#2{Algorithms \ref{#1} and \ref{#2}}
% Reference to a part, lower case
\def\partref#1{part~\ref{#1}}
% Reference to a part, upper case
\def\Partref#1{Part~\ref{#1}}
\def\twopartref#1#2{parts \ref{#1} and \ref{#2}}

\def\ceil#1{\lceil #1 \rceil}
\def\floor#1{\lfloor #1 \rfloor}
\def\1{\bm{1}}
\newcommand{\train}{\mathcal{D}}
\newcommand{\valid}{\mathcal{D_{\mathrm{valid}}}}
\newcommand{\test}{\mathcal{D_{\mathrm{test}}}}

\def\eps{{\epsilon}}


% Random variables
\def\reta{{\textnormal{$\eta$}}}
\def\ra{{\textnormal{a}}}
\def\rb{{\textnormal{b}}}
\def\rc{{\textnormal{c}}}
\def\rd{{\textnormal{d}}}
\def\re{{\textnormal{e}}}
\def\rf{{\textnormal{f}}}
\def\rg{{\textnormal{g}}}
\def\rh{{\textnormal{h}}}
\def\ri{{\textnormal{i}}}
\def\rj{{\textnormal{j}}}
\def\rk{{\textnormal{k}}}
\def\rl{{\textnormal{l}}}
% rm is already a command, just don't name any random variables m
\def\rn{{\textnormal{n}}}
\def\ro{{\textnormal{o}}}
\def\rp{{\textnormal{p}}}
\def\rq{{\textnormal{q}}}
\def\rr{{\textnormal{r}}}
\def\rs{{\textnormal{s}}}
\def\rt{{\textnormal{t}}}
\def\ru{{\textnormal{u}}}
\def\rv{{\textnormal{v}}}
\def\rw{{\textnormal{w}}}
\def\rx{{\textnormal{x}}}
\def\ry{{\textnormal{y}}}
\def\rz{{\textnormal{z}}}

% Random vectors
\def\rvepsilon{{\mathbf{\epsilon}}}
\def\rvtheta{{\mathbf{\theta}}}
\def\rva{{\mathbf{a}}}
\def\rvb{{\mathbf{b}}}
\def\rvc{{\mathbf{c}}}
\def\rvd{{\mathbf{d}}}
\def\rve{{\mathbf{e}}}
\def\rvf{{\mathbf{f}}}
\def\rvg{{\mathbf{g}}}
\def\rvh{{\mathbf{h}}}
\def\rvi{{\mathbf{i}}}
\def\rvj{{\mathbf{j}}}
\def\rvk{{\mathbf{k}}}
\def\rvl{{\mathbf{l}}}
\def\rvm{{\mathbf{m}}}
\def\rvn{{\mathbf{n}}}
\def\rvo{{\mathbf{o}}}
\def\rvp{{\mathbf{p}}}
\def\rvq{{\mathbf{q}}}
\def\rvr{{\mathbf{r}}}
\def\rvs{{\mathbf{s}}}
\def\rvt{{\mathbf{t}}}
\def\rvu{{\mathbf{u}}}
\def\rvv{{\mathbf{v}}}
\def\rvw{{\mathbf{w}}}
\def\rvx{{\mathbf{x}}}
\def\rvy{{\mathbf{y}}}
\def\rvz{{\mathbf{z}}}

% Elements of random vectors
\def\erva{{\textnormal{a}}}
\def\ervb{{\textnormal{b}}}
\def\ervc{{\textnormal{c}}}
\def\ervd{{\textnormal{d}}}
\def\erve{{\textnormal{e}}}
\def\ervf{{\textnormal{f}}}
\def\ervg{{\textnormal{g}}}
\def\ervh{{\textnormal{h}}}
\def\ervi{{\textnormal{i}}}
\def\ervj{{\textnormal{j}}}
\def\ervk{{\textnormal{k}}}
\def\ervl{{\textnormal{l}}}
\def\ervm{{\textnormal{m}}}
\def\ervn{{\textnormal{n}}}
\def\ervo{{\textnormal{o}}}
\def\ervp{{\textnormal{p}}}
\def\ervq{{\textnormal{q}}}
\def\ervr{{\textnormal{r}}}
\def\ervs{{\textnormal{s}}}
\def\ervt{{\textnormal{t}}}
\def\ervu{{\textnormal{u}}}
\def\ervv{{\textnormal{v}}}
\def\ervw{{\textnormal{w}}}
\def\ervx{{\textnormal{x}}}
\def\ervy{{\textnormal{y}}}
\def\ervz{{\textnormal{z}}}

% Random matrices
\def\rmA{{\mathbf{A}}}
\def\rmB{{\mathbf{B}}}
\def\rmC{{\mathbf{C}}}
\def\rmD{{\mathbf{D}}}
\def\rmE{{\mathbf{E}}}
\def\rmF{{\mathbf{F}}}
\def\rmG{{\mathbf{G}}}
\def\rmH{{\mathbf{H}}}
\def\rmI{{\mathbf{I}}}
\def\rmJ{{\mathbf{J}}}
\def\rmK{{\mathbf{K}}}
\def\rmL{{\mathbf{L}}}
\def\rmM{{\mathbf{M}}}
\def\rmN{{\mathbf{N}}}
\def\rmO{{\mathbf{O}}}
\def\rmP{{\mathbf{P}}}
\def\rmQ{{\mathbf{Q}}}
\def\rmR{{\mathbf{R}}}
\def\rmS{{\mathbf{S}}}
\def\rmT{{\mathbf{T}}}
\def\rmU{{\mathbf{U}}}
\def\rmV{{\mathbf{V}}}
\def\rmW{{\mathbf{W}}}
\def\rmX{{\mathbf{X}}}
\def\rmY{{\mathbf{Y}}}
\def\rmZ{{\mathbf{Z}}}

% Elements of random matrices
\def\ermA{{\textnormal{A}}}
\def\ermB{{\textnormal{B}}}
\def\ermC{{\textnormal{C}}}
\def\ermD{{\textnormal{D}}}
\def\ermE{{\textnormal{E}}}
\def\ermF{{\textnormal{F}}}
\def\ermG{{\textnormal{G}}}
\def\ermH{{\textnormal{H}}}
\def\ermI{{\textnormal{I}}}
\def\ermJ{{\textnormal{J}}}
\def\ermK{{\textnormal{K}}}
\def\ermL{{\textnormal{L}}}
\def\ermM{{\textnormal{M}}}
\def\ermN{{\textnormal{N}}}
\def\ermO{{\textnormal{O}}}
\def\ermP{{\textnormal{P}}}
\def\ermQ{{\textnormal{Q}}}
\def\ermR{{\textnormal{R}}}
\def\ermS{{\textnormal{S}}}
\def\ermT{{\textnormal{T}}}
\def\ermU{{\textnormal{U}}}
\def\ermV{{\textnormal{V}}}
\def\ermW{{\textnormal{W}}}
\def\ermX{{\textnormal{X}}}
\def\ermY{{\textnormal{Y}}}
\def\ermZ{{\textnormal{Z}}}

% Vectors
\def\vzero{{\bm{0}}}
\def\vone{{\bm{1}}}
\def\vmu{{\bm{\mu}}}
\def\vnu{{\bm{\nu}}}
\def\vtheta{{\bm{\theta}}}
\def\vgamma{{\bm{\gamma}}}
\def\vdelta{{\bm{\delta}}}
\def\vDelta{{\bm{\Delta}}}
\def\vepsilon{{\bm{\epsilon}}}
\def\va{{\bm{a}}}
\def\vb{{\bm{b}}}
\def\vc{{\bm{c}}}
\def\vd{{\bm{d}}}
\def\ve{{\bm{e}}}
\def\vehat{\bm{\hat{e}}}
\def\vetilde{\bm{\tilde{e}}}
\def\vell{{\bm{\ell}}}
\def\vf{{\bm{f}}}
\def\vfhat{{\bm{\hat{f}}}}
\def\vg{{\bm{g}}}
\def\vgtilde{\bm{\tilde{g}}}
\def\vghat{\bm{\hat{g}}}
\def\vh{{\bm{h}}}
\def\vi{{\bm{i}}}
\def\vj{{\bm{j}}}
\def\vk{{\bm{k}}}
\def\vl{{\bm{l}}}
\def\vm{{\bm{m}}}
\def\vmhat{{\bm{\hat{m}}}}
\def\vn{{\bm{n}}}
\def\vo{{\bm{o}}}
\def\vp{{\bm{p}}}
\def\vphi{{\bm{\phi}}}
\def\vq{{\bm{q}}}
\def\vr{{\bm{r}}}
\def\vs{{\bm{s}}}
\def\vstilde{\bm{\tilde{s}}}
\def\vt{{\bm{t}}}
\def\vu{{\bm{u}}}
\def\vv{{\bm{v}}}
\def\vvhat{{\bm{\hat{v}}}}
\def\vw{{\bm{w}}}
\def\vx{{\bm{x}}}
\def\vy{{\bm{y}}}
\def\vytilde{{\bm{\tilde{y}}}}
\def\vyhat{{\bm{\hat{y}}}}
\def\vz{{\bm{z}}}

% Elements of vectors
\def\evalpha{{\alpha}}
\def\evbeta{{\beta}}
\def\evepsilon{{\epsilon}}
\def\evlambda{{\lambda}}
\def\evomega{{\omega}}
\def\evmu{{\mu}}
\def\evpsi{{\psi}}
\def\evsigma{{\sigma}}
\def\evtheta{{\theta}}
\def\eva{{a}}
\def\evb{{b}}
\def\evc{{c}}
\def\evd{{d}}
\def\eve{{e}}
\def\evf{{f}}
\def\evg{{g}}
\def\evh{{h}}
\def\evi{{i}}
\def\evj{{j}}
\def\evk{{k}}
\def\evl{{l}}
\def\evm{{m}}
\def\evn{{n}}
\def\evo{{o}}
\def\evp{{p}}
\def\evq{{q}}
\def\evr{{r}}
\def\evs{{s}}
\def\evt{{t}}
\def\evu{{u}}
\def\evv{{v}}
\def\evw{{w}}
\def\evx{{x}}
\def\evy{{y}}
\def\evyhat{{\hat{y}}}
\def\evz{{z}}

% Matrix
\def\mA{{\bm{A}}}
\def\mB{{\bm{B}}}
\def\mC{{\bm{C}}}
\def\mD{{\bm{D}}}
\def\mE{{\bm{E}}}
\def\mF{{\bm{F}}}
\def\mG{{\bm{G}}}
\def\mGtilde{\bm{\tilde{G}}}
\def\mH{{\bm{H}}}
\def\mI{{\bm{I}}}
\def\mJ{{\bm{J}}}
\def\mK{{\bm{K}}}
\def\mL{{\bm{L}}}
\def\mM{{\bm{M}}}
\def\mN{{\bm{N}}}
\def\mO{{\bm{O}}}
\def\mP{{\bm{P}}}
\def\mQ{{\bm{Q}}}
\def\mR{{\bm{R}}}
\def\mS{{\bm{S}}}
\def\mT{{\bm{T}}}
\def\mU{{\bm{U}}}
\def\mV{{\bm{V}}}
\def\mW{{\bm{W}}}
\def\mWhat{{\bm{\hat{W}}}}
\def\mX{{\bm{X}}}
\def\mY{{\bm{Y}}}
\def\mZ{{\bm{Z}}}
\def\mBeta{{\bm{\beta}}}
\def\mPhi{{\bm{\Phi}}}
\def\mPi{{\bm{\Pi}}}
\def\mLambda{{\bm{\Lambda}}}
\def\mSigma{{\bm{\Sigma}}}
\def\mStilde{\bm{\tilde{\mS}}}
\def\mGtilde{\bm{\tilde{\mG}}}
\def\mGoverline{{\bm{\overline{G}}}}

% Tensor
\DeclareMathAlphabet{\mathsfit}{\encodingdefault}{\sfdefault}{m}{sl}
\SetMathAlphabet{\mathsfit}{bold}{\encodingdefault}{\sfdefault}{bx}{n}
\newcommand{\tens}[1]{\bm{\mathsfit{#1}}}
\def\tA{{\tens{A}}}
\def\tB{{\tens{B}}}
\def\tC{{\tens{C}}}
\def\tD{{\tens{D}}}
\def\tE{{\tens{E}}}
\def\tF{{\tens{F}}}
\def\tG{{\tens{G}}}
\def\tH{{\tens{H}}}
\def\tI{{\tens{I}}}
\def\tJ{{\tens{J}}}
\def\tK{{\tens{K}}}
\def\tL{{\tens{L}}}
\def\tM{{\tens{M}}}
\def\tN{{\tens{N}}}
\def\tO{{\tens{O}}}
\def\tP{{\tens{P}}}
\def\tQ{{\tens{Q}}}
\def\tR{{\tens{R}}}
\def\tS{{\tens{S}}}
\def\tT{{\tens{T}}}
\def\tU{{\tens{U}}}
\def\tV{{\tens{V}}}
\def\tW{{\tens{W}}}
\def\tX{{\tens{X}}}
\def\tY{{\tens{Y}}}
\def\tZ{{\tens{Z}}}


% Graph
\def\gA{{\mathcal{A}}}
\def\gB{{\mathcal{B}}}
\def\gC{{\mathcal{C}}}
\def\gD{{\mathcal{D}}}
\def\gE{{\mathcal{E}}}
\def\gF{{\mathcal{F}}}
\def\gG{{\mathcal{G}}}
\def\gH{{\mathcal{H}}}
\def\gI{{\mathcal{I}}}
\def\gJ{{\mathcal{J}}}
\def\gK{{\mathcal{K}}}
\def\gL{{\mathcal{L}}}
\def\gM{{\mathcal{M}}}
\def\gN{{\mathcal{N}}}
\def\gO{{\mathcal{O}}}
\def\gP{{\mathcal{P}}}
\def\gQ{{\mathcal{Q}}}
\def\gR{{\mathcal{R}}}
\def\gS{{\mathcal{S}}}
\def\gT{{\mathcal{T}}}
\def\gU{{\mathcal{U}}}
\def\gV{{\mathcal{V}}}
\def\gW{{\mathcal{W}}}
\def\gX{{\mathcal{X}}}
\def\gY{{\mathcal{Y}}}
\def\gZ{{\mathcal{Z}}}

% Sets
\def\sA{{\mathbb{A}}}
\def\sB{{\mathbb{B}}}
\def\sC{{\mathbb{C}}}
\def\sD{{\mathbb{D}}}
% Don't use a set called E, because this would be the same as our symbol
% for expectation.
\def\sF{{\mathbb{F}}}
\def\sG{{\mathbb{G}}}
\def\sH{{\mathbb{H}}}
\def\sI{{\mathbb{I}}}
\def\sJ{{\mathbb{J}}}
\def\sK{{\mathbb{K}}}
\def\sL{{\mathbb{L}}}
\def\sM{{\mathbb{M}}}
\def\sN{{\mathbb{N}}}
\def\sO{{\mathbb{O}}}
\def\sP{{\mathbb{P}}}
\def\sQ{{\mathbb{Q}}}
\def\sR{{\mathbb{R}}}
\def\sS{{\mathbb{S}}}
\def\sT{{\mathbb{T}}}
\def\sU{{\mathbb{U}}}
\def\sV{{\mathbb{V}}}
\def\sW{{\mathbb{W}}}
\def\sX{{\mathbb{X}}}
\def\sY{{\mathbb{Y}}}
\def\sYhat{{\hat{\mathbb{Y}}}}
\def\sZ{{\mathbb{Z}}}
% Blackboard Greek characters: https://tex.stackexchange.com/a/3260
\DeclareSymbolFont{bbold}{U}{bbold}{m}{n}
\DeclareSymbolFontAlphabet{\mathbbold}{bbold}
\def\sOmega{{\mathbbold{\Omega}}}
\def\sPhi{{\mathbbold{\Phi}}}
\def\sTheta{{\mathbbold{\Theta}}}

% Entries of a matrix
\def\emLambda{{\Lambda}}
\def\emA{{A}}
\def\emB{{B}}
\def\emC{{C}}
\def\emD{{D}}
\def\emE{{E}}
\def\emF{{F}}
\def\emG{{G}}
\def\emH{{H}}
\def\emI{{I}}
\def\emJ{{J}}
\def\emK{{K}}
\def\emL{{L}}
\def\emM{{M}}
\def\emN{{N}}
\def\emO{{O}}
\def\emP{{P}}
\def\emQ{{Q}}
\def\emR{{R}}
\def\emS{{S}}
\def\emT{{T}}
\def\emU{{U}}
\def\emV{{V}}
\def\emW{{W}}
\def\emX{{X}}
\def\emY{{Y}}
\def\emZ{{Z}}
\def\emSigma{{\Sigma}}
\def\emPi{{\Pi}}

% entries of a tensor
% Same font as tensor, without \bm wrapper
\newcommand{\etens}[1]{\mathsfit{#1}}
\def\etLambda{{\etens{\Lambda}}}
\def\etA{{\etens{A}}}
\def\etB{{\etens{B}}}
\def\etC{{\etens{C}}}
\def\etD{{\etens{D}}}
\def\etE{{\etens{E}}}
\def\etF{{\etens{F}}}
\def\etG{{\etens{G}}}
\def\etH{{\etens{H}}}
\def\etI{{\etens{I}}}
\def\etJ{{\etens{J}}}
\def\etK{{\etens{K}}}
\def\etL{{\etens{L}}}
\def\etM{{\etens{M}}}
\def\etN{{\etens{N}}}
\def\etO{{\etens{O}}}
\def\etP{{\etens{P}}}
\def\etQ{{\etens{Q}}}
\def\etR{{\etens{R}}}
\def\etS{{\etens{S}}}
\def\etT{{\etens{T}}}
\def\etU{{\etens{U}}}
\def\etV{{\etens{V}}}
\def\etW{{\etens{W}}}
\def\etX{{\etens{X}}}
\def\etY{{\etens{Y}}}
\def\etZ{{\etens{Z}}}

\newcommand{\pdf}{p}

% The true underlying data generating distribution
\newcommand{\pdata}{p_{\mathrm{data}}}
% The empirical distribution defined by the training set
\newcommand{\ptrain}{\hat{p}_{\mathrm{data}}}
\newcommand{\Ptrain}{\hat{P}_{\mathrm{data}}}
% The model distribution
\newcommand{\pmodel}{p_{\rm{model}}}
\newcommand{\Pmodel}{P_{\rm{model}}}
\newcommand{\ptildemodel}{\tilde{p}_{\rm{model}}}
% Stochastic autoencoder distributions
\newcommand{\pencode}{p_{\rm{encoder}}}
\newcommand{\pdecode}{p_{\rm{decoder}}}
\newcommand{\precons}{p_{\rm{reconstruct}}}

\ifcsname laplace\endcsname%
    \renewcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\else%
    \newcommand{\laplace}{\mathrm{Laplace}}% Laplace distribution
\fi

%\newcommand{\E}{\mathbb{E}}
%\DeclareMathOperator{\E}{\mathbb{E}}

\newcommand{\Ls}{\mathcal{L}}
%\newcommand{\R}{\mathbb{R}}
\newcommand{\emp}{\tilde{p}}
\newcommand{\lr}{\alpha}
\newcommand{\reg}{\lambda}
\newcommand{\rect}{\mathrm{rectifier}}
\newcommand{\softmax}{\mathrm{softmax}}
\newcommand{\onehot}{\mathrm{onehot}}
\newcommand{\sigmoid}{\sigma}
\newcommand{\softplus}{\zeta}
%\newcommand{\KL}{D_{\mathrm{KL}}}
%\DeclareMathOperator{\KL}{KL}
%\newcommand{\Var}{\mathrm{Var}}
\newcommand{\standarderror}{\mathrm{SE}}
\newcommand{\Cov}{\mathrm{Cov}}
% Wolfram Mathworld says $L^2$ is for function spaces and $\ell^2$ is for vectors
% But then they seem to use $L^2$ for vectors throughout the site, and so does
% wikipedia.
\newcommand{\normlzero}{L^0}
\newcommand{\normlone}{L^1}
\newcommand{\normltwo}{L^2}
\newcommand{\normlp}{L^p}
\newcommand{\normmax}{L^\infty}

%\newcommand{\parents}{Pa} % See usage in notation.tex. Chosen to match Daphne's book.

% \newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}_{#1}}\xspace}}
% \newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}_{#1}}\xspace}}
% \newcommand{\children}[1]{{\ensuremath{\mathrm{ch}_{#1}}\xspace}}

\newcommand{\parents}[1]{{\ensuremath{\mathrm{pa}(#1)}\xspace}}
\newcommand{\ancestors}[1]{{\ensuremath{\mathrm{an}(#1)}\xspace}}
\newcommand{\children}[1]{{\ensuremath{\mathrm{ch}(#1)}\xspace}}

%\DeclareMathOperator*{\argmax}{arg\,max}
%\DeclareMathOperator*{\argmin}{arg\,min}
%\DeclareMathOperator*{\minimize}{minimize}
%\DeclareMathOperator*{\maximize}{maximize}

\DeclareMathOperator{\sign}{sign}
%\DeclareMathOperator{\mean}{mean}
\DeclareMathOperator{\vmap}{vmap}
\DeclareMathOperator{\reshape}{reshape}
%\DeclareMathOperator{\Tr}{Tr}
\DeclareMathOperator{\diag}{diag}
\DeclareMathOperator{\eig}{eig}
\DeclareMathOperator{\rank}{rank}
\DeclareMathOperator{\vecspan}{span}
\DeclareMathOperator{\overlap}{overlap}
\DeclareMathOperator{\Cat}{Cat}

%%%%% NEW MATH DEFINITIONS %%%%%
\newcommand{\grad}[1]{\ensuremath{\nabla_{\!{#1}}}}
\newcommand{\naturalgrad}[1]{\ensuremath{\tilde{\nabla}_{\!{#1}}}}
\newcommand{\gradsquared}[1]{\ensuremath{\nabla_{\!{#1}}^{2}}}
\newcommand{\hess}[1]{\ensuremath{\mathrm{H}_{#1}}}

\newcommand{\Dtrain}{\ensuremath{\sD_{\mathrm{train}}}}
\newcommand{\Dtest}{\ensuremath{\sD_{\mathrm{test}}}}
\newcommand{\Dvalid}{\ensuremath{\sD_{\mathrm{valid}}}}


% || for KLDivergence
\DeclarePairedDelimiterX{\KLdivx}[2]{(}{)}{%
  #1\;\delimsize\|\;#2%
}
\newcommand{\KLdiv}{\KL\KLdivx}

\NewDocumentCommand{\giventhat}{O{\;|} m m}{#2#1\;#3}

\let\ab\allowbreak


%%% Local Variables:
%%% mode: latex
%%% TeX-master: "../thesis"
%%% End:


==> my_commands.tex <==

%%% Colors
\colorlet{idcolor}{greendark}
\colorlet{unidcolor}{SBred}
\colorlet{hiddencolor}{gray}

\newcommand{\maincolor}{\textcolor{maincolor}{blue}\xspace}
\newcommand{\Maincolor}{\textcolor{maincolor}{Blue}\xspace}
\let\firstcolor\maincolor
\let\Firstcolor\Maincolor
\newcommand{\secondcolor}{\textcolor{secondcolor}{red}\xspace}
\newcommand{\Secondcolor}{\textcolor{secondcolor}{Red}\xspace}

%%% Boxes

\newtcolorbox{takeaway}{
    colback=maincolor!5!white, colframe=maincolor!75!black
}

%%% Text

\newcommand{\methodname}[1]{\texttt{\small #1}}


%%%

\newcommand{\oursIcon}{\faMicrochip\xspace}
% \newcommand{\ours}{TORO\xspace} % TODO change
% \newcommand{\Ours}{TORO\xspace}
\newcommand{\our}{{causalKAN} \xspace}
\newcommand{\Our}{{CausalKAN} \xspace}
\newcommand{\ours}{{causalKANs}\xspace} % TODO change
\newcommand{\Ours}{{CausalKANs}\xspace}
% \newcommand{\ourspl}{\textit{Decafs}\xspace} % TODO change
% \newcommand{\Ourspl}{\textit{Decaf}\xspace}
% \newcommand{\ourslong}{my model long\xspace}

\newcommand{\skan}{S-KAN \xspace}
\newcommand{\tkan}{T-KAN \xspace}
\newcommand{\tarkan}{TARKAN \xspace}
\newcommand{\dragonkan}{DragonKAN \xspace}


\newcommand{\eqcomment}[1]{\text{[\textit{#1}]}}

%\renewcommand{\itemi}{\textit{i)}\xspace}
%\renewcommand{\itemii}{\textit{ii)}\xspace}
%\renewcommand{\itemiii}{\textit{iii)}\xspace}
%\renewcommand{\itemiv}{\textit{iv)}\xspace}
%\renewcommand{\itemv}{\textit{v)}\xspace}
%\newcommand{\itemvi}{\textit{vi)}\xspace}
%\newcommand{\itemvii}{\textit{vii)}\xspace}

%%% SYMBOLS

\newcommand{\kanlayer}{\ensuremath{\phi}\xspace}
\newcommand{\kanoutlayer}{\ensuremath{\Phi}\xspace}
\newcommand{\kan}{\ensuremath{\boldsymbol\Phi}\xspace}
\newcommand{\ELBO}{\ensuremath{\mathcal{L}}\xspace}

\newcommand{\splinecoef}{\ensuremath{w_s}\xspace}
\newcommand{\splinebiascoef}{\ensuremath{w_b}\xspace}
\newcommand{\weight}{\ensuremath{\lambda}\xspace}

%\let\pred\tilde
\renewcommand{\cond}[1]{{|{#1}}}
\newcommand{\pred}[1]{\ensuremath{\tilde{#1}}\xspace}
\newcommand{\factual}[1]{\ensuremath{{#1}^\text{\normalfont{f}}}}
\newcommand{\cfactual}[1]{\ensuremath{{#1}^\text{\normalfont{cf}}}}

\newcommand{\indexone}{\ensuremath{i}\xspace}
\newcommand{\indextwo}{\ensuremath{j}\xspace}
\newcommand{\indexthree}{\ensuremath{q}\xspace}
\newcommand{\indexfour}{\ensuremath{k}\xspace}
\newcommand{\indexlayer}{\ensuremath{l}\xspace}
\newcommand{\indexfive}{\ensuremath{r}\xspace}
\newcommand{\indexsix}{\ensuremath{s}\xspace}

\newcommand{\nLayers}{\ensuremath{L}\xspace}

\newcommand{\query}{\ensuremath{Q}\xspace}

\newcommand{\doop}{\text{do}}


\newcommand{\scmfamily}{\ensuremath{\mathbb{M}}\xspace}
\newcommand{\scm}{\ensuremath{\mathcal{M}}\xspace}
\newcommand{\graph}{\ensuremath{\mathcal{G}}\xspace}
\newcommand{\func}[1][]{\ensuremath{f_{#1}}\xspace}
\newcommand{\funcb}[1][]{\ensuremath{\mathbf{g}_{#1}}\xspace}
\newcommand{\predfuncb}[1][]{\ensuremath{{\pred{\mathbf{f}}}_{#1}}\xspace}
\newcommand{\functrue}[1][]{\ensuremath{f^\star_{#1}}\xspace}

\newcommand{\functionclass}[1][]{\ensuremath{\mathcal{F}}\xspace}

% \newcommand{\varparents}[2][\varobs]{\ensuremath{{#1}_\parents{#2}}\xspace}
\newcommand{\varparents}[2][\varobs]{\ensuremath{\parents{#2}}\xspace}
% \newcommand{\varchildren}[2][\varobs]{\ensuremath{{#1}_\children{#2}}\xspace}
\newcommand{\varchildren}[2][\varobs]{\ensuremath{\children{#2}}\xspace}

\newcommand{\edist}{\ensuremath{\tilde{p}}\xspace}

\newcommand{\outcome}{\ensuremath{\rvy}\xspace}
\newcommand{\treatment}{\ensuremath{\rvt}\xspace}
\newcommand{\covariates}
{\ensuremath{\rvx}\xspace}
\newcommand{\covariate}
{\ensuremath{\text{x}}\xspace}
\newcommand{\latent}{\ensuremath{\rvz}\xspace}
\newcommand{\exogenous}{\ensuremath{\rvu}\xspace}

% \newcommand{\timepoint}{\ensuremath{\tau}\xspace}
% \newcommand{\timevar}{\ensuremath{\taub}\xspace}

\newcommand{\ite}{\ensuremath{\tau_\indexone}\xspace}
\newcommand{\cate}[1]{\ensuremath{\tau}(#1)\xspace}
\newcommand{\ate}{\ensuremath{\tau}\xspace}
\newcommand{\hcate}[1]{\ensuremath{\hat{\tau}}(#1)\xspace}


\newcommand{\hazard}{\ensuremath{h}\xspace}
\newcommand{\survival}{\ensuremath{S}\xspace}

\newcommand{\dataset}{\ensuremath{\mathcal{D}}\xspace}

\newcommand{\samplecov}{\ensuremath{\vx}\xspace}
\newcommand{\samplecovi}{\ensuremath{x}\xspace}
\newcommand{\samplelatent}{\ensuremath{\vz}\xspace}
\newcommand{\samplelatenti}{\ensuremath{z}\xspace}
\newcommand{\sampletreat}{\ensuremath{t}\xspace}
\newcommand{\sampletreati}{\ensuremath{t}\xspace}
\newcommand{\sampleoutcome}{\ensuremath{y}\xspace}
\newcommand{\sampleoutcomei}{\ensuremath{y}\xspace}

\newcommand{\samplekan}{\samplelatenti}

\newcommand{\covspace}{\ensuremath{\mathcal{X}}\xspace}
\newcommand{\treatmentspace}{\ensuremath{\mathcal{T}}\xspace}

\newcommand{\numtreatments}{\ensuremath{K}\xspace}

% \newcommand{\obssize}{\ensuremath{{D_\rvx}}\xspace}
\newcommand{\covsize}{\ensuremath{{D}}\xspace}
\newcommand{\latentsize}{{\ensuremath{\covsize_\latent}}\xspace}
\newcommand{\samplesize}{\ensuremath{N}\xspace}
\newcommand{\allsize}{\ensuremath{{D_\rvv}}\xspace}
\newcommand{\proxysize}{\ensuremath{{S}}\xspace}

\newcommand{\leftedge}{L\xspace}
\newcommand{\rightedge}{R\xspace}
\newcommand{\presence}[1]{\textcolor{firstcolor}{#1}}
\newcommand{\absence}[1]{\textcolor{secondcolor}{#1}}

\newcommand{\pozero}{\ensuremath{\mu_0}\xspace}
\newcommand{\hpozero}{\ensuremath{\hat{\mu}_0}\xspace}
\newcommand{\poone}{\ensuremath{\mu_1}\xspace}
\newcommand{\hpoone}{\ensuremath{\hat{\mu}_1}\xspace}
\newcommand{\pot}{\ensuremath{\mu_\sampletreati}\xspace}
\newcommand{\hpot}{\ensuremath{\hat{\mu}_\sampletreati}\xspace}
\newcommand{\propensity}{\ensuremath{e}\xspace}
\newcommand{\hpropensity}{\ensuremath{\hat{\propensity}}\xspace}
\newcommand{\hpo}{\ensuremath{\hat{\mu}}\xspace}

\newcommand{\score}{\ensuremath{s}\xspace}
\newcommand{\threshold}{\ensuremath{\Gamma}\xspace}
\newcommand{\budget}{\ensuremath{\Lambda}\xspace}

\newcommand{\significancelevel}{\ensuremath{\alpha}\xspace}
\newcommand{\regularization}{\ensuremath{\mathcal{R}}\xspace}

\newcommand{\representationspace}{\ensuremath{\boldsymbol\Delta}\xspace}

\newcommand{\pottrue}{\ensuremath{\mu^\star_\sampletreati}\xspace}
\newcommand{\pozerotrue}{\ensuremath{\mu^\star_0}\xspace}
\newcommand{\poonetrue}{\ensuremath{\mu^\star_1}\xspace}


% CATE additive components (true and estimated)
\newcommand{\catecomp}[1]{\ensuremath{\tau_{#1}}\xspace}
\newcommand{\hcatecomp}[1]{\ensuremath{\hat{\tau}_{#1}}\xspace}

% Risk functional
\newcommand{\risk}{\ensuremath{R}\xspace}

% Additive residual functions used in the identifiability proof
\newcommand{\addresid}{\ensuremath{h}\xspace}
\newcommand{\addresidc}{\ensuremath{\tilde{h}}\xspace}

% Additive constants in the decompositions
\newcommand{\addconst}{\ensuremath{a}\xspace}
\newcommand{\const}{\ensuremath{c}\xspace}

==> tikz.tex <==
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% LIBRARIES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
\usetikzlibrary{
    shapes,
    pgfplots.groupplots,
    shadings,
    calc,
    arrows,
    backgrounds,
    colorbrewer,
    shadows.blur,
    external,
    shapes,
    shapes.arrows,
    shapes.symbols,
    arrows.meta,
    positioning, 
    decorations.pathreplacing,
    intersections,
    cd,
    scopes,
    babel, % otherwise there is an error when importing spanish in babel
    fit % For extending the bounding box
}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% STYLES
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%\tikzset{every picture/.style={->, shorten >=1pt, thick}}

% in preamble
\tikzcdset{
    nodes={anchor=center},
    arrow style=tikz,
    diagrams={>={Stealth[scale=0.8]}},
%    diagrams={>={Straight Barb[scale=0.8]}},
}

% \tikzstyle{main node}=[circle,draw,font=\sffamily\Large\bfseries]
\tikzstyle{main node}=[circle,draw,font=\sffamily\small,inner sep=0pt, outer sep=0pt, minimum size=5mm]
\tikzstyle{observed}=[style=main node, fill=gray!25]
\tikzstyle{hidden}=[style=main node, fill=white, dashed, draw=black!40, text=black!60]
\tikzstyle{hiddenarrow}=[dashed, draw=black!40]
\tikzstyle{realobs}=[style=main node,  ellipse]
\tikzstyle{realhidden}=[style=hidden, ellipse]
\tikzstyle{fairnessobs} = [style=main node, ellipse, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzstyle{fairnesshidden} = [style=main node, ellipse, fill=white, dashed, draw=black!60, text=black!60, minimum height=5mm,minimum width=10mm] %Ellipse for fairness
\tikzset{
    given variable/.style = {
        draw=none, outer sep=0pt, inner sep=0pt, "#1"{yshift=-5pt}
    }
}

\tikzstyle{identifiable}=[draw=idcolor, very thick]
\tikzstyle{nonidentifiable}=[draw=unidcolor, very thick]


\tikzstyle{block} = [rectangle, draw, minimum width=0.5 cm, minimum height=1.5cm]
\tikzstyle{cir} = [circle, draw, minimum size=0.3cm]
\tikzstyle{startstop} = [rectangle, rounded corners, minimum width=3cm, minimum height=1cm,text centered, draw=black]
\tikzstyle{process} = [rectangle, minimum width=3cm, minimum height=1cm, text centered, draw=black]
\tikzstyle{decision} = [diamond, aspect=2.5, minimum width=3cm, text centered, draw=black]
\tikzstyle{arrow} = [thick,->,>=stealth]
\tikzstyle{hexa} = [trapezium, trapezium left angle=60, trapezium right angle=120, draw,  
      minimum width=2cm, minimum height=0.5cm]


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%% Other commands
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\newcommand\irregularcircle[2]{% radius, irregularity
    \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
    +(0:\len pt)
    \foreach \a in {10,20,...,350}{
        \pgfextra {\pgfmathsetmacro\len{(#1)+rand*(#2)}}
        -- +(\a:\len pt)
    } -- cycle
}


\pgfdeclareplotmark{mystar}{
    \node[star,star point ratio=2.25,minimum size=6pt,
    inner sep=0pt,draw=black,solid,fill=red] {};
}

% Optional: tighter spacing inside nodes
\newcommand{\nodew}{50mm}  % tweak node width
